Emotion and Sentiment Guided Paraphrasing

Paraphrase generation, a.k.a. paraphrasing, is a common and important task in natural language processing. Emotional paraphrasing, which changes the emotion embodied in a piece of text while preserving its meaning, has many potential applications, including moderating online dialogues and preventing cyberbullying. We introduce a new task of fine-grained emotional paraphrasing along emotion gradients, that is, altering the emotional intensities of the paraphrases in fine-grained settings following smooth variations in affective dimensions while preserving the meaning of the original text. We reconstruct several widely used paraphrasing datasets by augmenting the input and target texts with their fine-grained emotion labels. Then, we propose a framework for emotion and sentiment guided paraphrasing by leveraging pre-trained language models for conditioned text generation. Extensive evaluation of the fine-tuned models suggests that including fine-grained emotion labels in the paraphrase task significantly improves the likelihood of obtaining high-quality paraphrases that reflect the desired emotions while achieving consistently better scores in paraphrase metrics such as BLEU, ROUGE, and METEOR.

==> emo-transition.tex <==
\subsection{Emotion Transition Testing}
Up until this point in the paper, the evaluations that have been executed have involved testing the emotion paraphrasing potential of the trained models. However, a crucial aspect of the proposed model involves an emotion-transition graph with emotion gradients.

==> extra_stuff.tex <==

%your original detailed write up Section 2 in case you need it later 




\subsection{Emotion Psychology and Classification}
Emotions are a key component of human psychology. 
They play a role in many cognitive processes including learning, memory, decision making, and interpersonal communication \citep{oatley1994experience, tyng2017influences}. 
Emotions dictate the context and mood by which memories are formed. 
They guide our conscious actions and our body’s unconscious processes. 
An emotion like fear signals the Sympathetic Nervous System to constrict blood vessels, dilate the pupils, and increase the heart rate \citep{alshak2019neuroanatomy}. 
Emotions connect the body’s systems and one’s thoughts towards what is triggering the intense flow of emotions \citep{oatley1994experience}.

Equally important is the role that emotions play in human-to-human interactions. 
%Facial expressions, for example, are an integral part of interpersonal interactions. 
%A small shift in the lips, the eyebrows, or the forehead can signal different emotions to humans who have an innate ability to recognize other human-displayed emotions \citep{frith2009role}. 
Small intonation changes and a rise and lowering of the pitch in one's voice can also signal different emotions \citep{tiwari2012voice}. 
The quick registration of emotions by the body’s senses is efficient for communication. However, 
because emotions act as “heuristics” for the human body \citep{oatley1994experience}, 
it is also quick, and often too quick, to offend in its response in communication. 
Words can trigger emotional responses, both negative and positive. 
Words and languages have been shown to play a key role in helping people distinguish the emotions they feel \citep{lindquist2015role}.

In the Internet age, where 72\% of United States adults are on social media ~\citep{pewresearch2022socialmediafactsheet},
the importance of words in communication has grown. 
Without facial expressions, vocal intonations, or hand gestures, 
it is harder to communicate one’s emotions online. 
The intensities of words can be misinterpreted or be higher than what someone wants them to communicate. 
For example, 
someone could want to communicate frustration, but instead could come off as furious. 
Rooted in the psychology of communication and emotion, the need for lowering the intensity of online communications inspires the task of fine-grained emotion-paraphrasing along emotion gradients.

\begin{comment}
\subsection{Sentiment Analysis} 
Sentiment analysis is the NLP task of finding the opinion, attitude, or view of a given input text. 
One sub task of sentiment analysis is the polarity classification which involves classifying the text into one of three basic categories: positive, negative, and neutral. This can be done through supervised learning, a lexicon-based approach, or a hybrid of the two \citep{sadia2018overview}. 
Polarity classification has been done on a variety of sentence types such as reviews \citep{turney2002thumbs, pang2002thumbs}, conditional sentences \citep{narayanan2009sentiment}, and Tweets \citep{pak2010twitter}.
However, 
polarity classification does not allow detailed identification of emotions that is necessary for emotional paraphrasing. 
Emotion classification is needed for this task.
\end{comment}

\subsection{Emotion Classification}
In 1890, \citeauthor{james1890principles}
proposed fear, grief, love, and rage as a set of the most basic emotions. 
Then in 1992, 
Paul Ekman introduced his famous set of six basic emotions: fear, anger, joy, sadness, disgust, and surprise \citep{ekman1992argument}. 
They are the basis of many emotional psychology studies and NLP experiments pertaining to emotions. 
Another classification produced by \citeauthor{lazarus1994passion} included a list of 15 emotions. 
Recently a study done by \citeauthor{cowen2017self} expanded on these classifications. 
By having human test subjects report on the emotions they felt while viewing videos, 
the study found that there were 27 emotion categories, in addition to a neutral emotion. 
This study also grouped these emotions into ``clusters.''

\citet{demszky2020goemotions} produced a similar set of 28 emotions that was used in the GoEmotions project. 
This project provided a labeled dataset of 58k texts and a BERT-based machine learning model capable of classifying inputs into one of the 28 emotions. 
In addition, 
the GoEmotions project provided a heat map showing the correlation between emotions as well as including a stratification of the emotions into clusters as shown in Table~\ref{EmotionClusters}. 
% As we planned to leverage the GoEmotions model to classify our texts, 
% we used the 28 emotions that were used in the GoEmotions project, 
% modeling our clusters after the clustering map provided in the study that originally reported finding the 28 emotions. 
These clusters provided guidance for how our emotion-transition graph can be structured. 

\begin{table}[h!]

\centering
%\def\arraystretch{1.5}
\small
\begin{tabular}{ c | l }
\hline
\textbf{Group} & \textbf{Emotions} \\
\hline
 1 & Neutral \\
 2 & Amusement, Excitement, Joy, Love \\
 3 & Optimism, Desire, Caring \\
 4 & Pride, Admiration \\
 5 & Gratitude, Relief \\
 6 & Approval, Realization \\
 7 & Surprise, Curiosity, Confusion \\
 8 & Fear, Nervousness \\
 9 & Remorse, Embarrassment \\ 
 10 & Disappointment, Sadness, Grief \\
 11 & Disgust, Anger, Annoyance, Disapproval
\end{tabular}
\caption{Emotion Grouping by \citet{demszky2020goemotions}}
\label{EmotionClusters} 
\end{table}


\begin{comment}
\subsection{Transformers in Natural Language Generation} Natural Language Generation (NLG) include tasks such as summarization, translation, chatbots, question generation, long text generation, and paraphrase generation \citep{celikyilmaz2020evaluation}. 
One of the breakthrough NLG models is the Transformer model \citep{vaswani2017attention}, which utilizes the mechanism of self-attention: differentially weighting the significance of different parts of the input data. Bidirectional Encoder Representations from Transformers (BERT) is a well-known language model based on Transformers and pretrained for two tasks: language modeling and next sentence generation~\citep{devlin2018bert}. The GoEmotions' emotion classification model is based on BERT. One of the most complex Transformer-based models is Generative Pre-trained Transformer (GPT), an autoregressive language model. Both of its recent editions, GPT-2~\citep{radford2019language} and GPT-3~\citep{brown2020gpt3} were trained with a dataset containing billions of parameters capable of a wide variety of tasks.

Text-to-text Transformer models such as Bart \citep{lewis2019bart} and T5  \citep{raffel2020exploring} are Transformer models following the text-to-text approach. They provide a high level of flexibility in NLG tasks because many problems can be solved by a text-to-text Transformer model through similar training or fine-tuning methods. Both Bart and T5 use the standard encoder-decoder Transformer model. 
BART utilizes a technique called ``denoising" for pretraining sequence-to-sequence models based on a combination of Bidirectional and Auto-Regressive Transformers, while
T5 was developed through a process of transfer learning. 
Transfer learning involves training the model on a vast set of wide-ranging data with the goal of being able to use the model on a multitude of ``downstream" tasks. 
The T5 model accepts an optional ``prefix" before the input to specify the task.
A sample input, as provided by \citeauthor{raffel2020exploring}, involves the translation of text from English to German. 
In this example, 
T5 would take the input as ``translate English to German: (text to be translate)." 
This flexibility allowed us to use our input and target emotions as the prefixes in  fine-tuning T5 for implementing the task of fine-grained emotional-paraphrasing.
\end{comment}



\subsection{Paraphrasing} 
Paraphrasing is a key task in the NLG domain. It involves inputting text and returning one of similar meaning. 
Approaches to paraphrasing include the use of sentence pattern and feature statistics \citep{zhao2009application}, 
repurposing unsupervised style transfer \citep{krishna2020reformulating},
imitation and reinforcement learning \citep{du2019empirical},
a latent bag-of-words \citep{fu2019paraphrase},
and pointer-generator networks \citep{see2017get}.
Several models combine deep generative models with other modeling and training techniques:  
e.g., variations using reinforcement learning \citep{li2017paraphrase},
long short-term memory or LSTM \citep{gupta2018deep}, 
and stacked residual LSTM \citep{prakash2016neural}.
Other approaches focus on specific variations of paraphrasing. 
These include using reinforcement learning for the multi-paraphrase generation \citep{qian2019exploring}, weakly supervised learning for entailment-relation-aware paraphrasing \citep{sancheti2022entailment},
adversarial training for end-to-end paraphrasing \citep{yang2019end},
and syntax-guidance for guided paraphrasing \citep{kumar2020syntax}.

Transformer-based text-to-text models such as BART \citep{lewis2019bart} and T5 \citep{raffel2020exploring} have become more popular for use in paraphrasing. 
Several studies have been done to improve these models' paraphrasing performance through joint paraphrase learning \citep{min2020advancing},
topic-focused training \citep{liu2019generating},
and combining copying and generative decoders \citep{cao2017joint}. Work has also been done to combine Transformers and seq2seq models to improve paraphrase generation \citep{egonmwan2019transformer}.

%Equally important to paraphrasing is the evaluation of paraphrase quality. The most common metrics used for paraphrase evaluation are BLEU \citep{papineni2002bleu}, ROUGE \citep{lin2004rouge}, and METEOR \citep{banerjee2005meteor}. Recently, newer scores have also been proposed for evaluating text generation and paraphrase models include Google BLEU \citep{wu2016google} - a variation of the classic BLEU score, the BERTScore \citep{zhang2019bertscore} - obtained using the BERT model,  MAUVE \citep{pillutla2021mauve}, BBScore \citep{shen2022revisiting}, and fine-grained pair-wise word interactions (PWI) scores \citep{he2016pairwise}.


Emotional paraphrasing is a task that has been closely studied.
In \citep{casas2021emotional}, GPT models were utilized for 
emotional paraphrasing. Input text was paraphrased to fit 
one of Ekman's six emotional categories. Six fine-tuned 
GPT models (one for each emotion) are utilized to ``enhance" the 
emotion of the input text which was then paraphrased. While 
our task shares similar goal in emotional paraphrasing, 
our fine-grained paraphrasing solution is more flexible. It utilizes a more fine-grained emotion categorization, conducts
emotional transition based on the emotion of the input text,  
and is capable of transitioning to various emotions along 
emotion gradients on a transition graph.  

% While their task is similar to emotional paraphrasing along 
% emotion gradients, our solution utilizes one model and a 
% transition-graph to generate a emotionally paraphrased output. 
% Our proposed solution is capable of classifying to solution 
% before lowering its emotional intensity. This makes our model flexible, 
% as opposed to the model proposed by \citeauthor{casas2021emotional}. 
% Our model decides what emotion to paraphrase to based on the input, 
% while their GPT model outputs all six variations of text that 
% represent all of the emotion spectrum.

As our task lowers emotional intensity of input texts, and 
thereby lowering the strong psychological effects that intense 
emotional interactions can bring, it relates to the task 
of positive reframing \citep{ziems2022inducing}. Both focus on 
altering the emotions of texts, while preserving its 
underlying connotations. However, the task of positive 
reframing emphasized altering the input text into a positive 
emotion while our task does not translate every emotion into 
a positive one, but rather lowers the intensity of emotions, 
which allows negative and positive emotions alike.

Our goal of lowering the intensity of emotions in text is 
related to, but different from the task of neutralizing bias \citep{pryzant2020automatically}. Neutralizing bias strives to eliminate all bias, which results in most paraphrased texts being classified as \textit{neutral}. In our task of emotion paraphrasing along emotion-gradients, we aim to preserve the base meaning and tone while lowering the intensity of the input text. Thus, the text still expresses its original view or 
belief,  but in a less provocative or intense manner.
